Coalescing Global and Local Information for Procedural Text Understanding

Procedural text understanding is a challenging language reasoning task that requires models to track entity states across the development of a narrative. A complete procedural understanding solution should combine three core aspects: local and global views of the inputs, and global view of outputs. Prior methods considered a subset of these aspects, resulting in either low precision or low recall. In this paper, we propose Coalescing Global and Local Information (CGLI), a new model that builds entity- and timestep-aware input representations (local input) considering the whole context (global input), and we jointly model the entity states with a structured prediction objective (global output). Thus, CGLI simultaneously optimizes for both precision and recall. We extend CGLI with additional output layers and integrate it into a story reasoning framework. Extensive experiments on a popular procedural text understanding dataset show that our model achieves state-of-the-art results; experiments on a story reasoning benchmark show the positive impact of our model on downstream reasoning.

==> Approach_old.tex <==
\section{Approaches}

%\filip{one way to save space in sec 2+3 is to transform the subsections into textbf inline headers.}
In this section, we formally define the tasks we consider in \autoref{subsec:task1}. Then we describe the proposed method in \autoref{subsec:input}-\autoref{subsec:train}. We describe specific adaptations for story understanding in \autoref{subsec:adapt}. Our proposed model is shown in \autoref{fig:model}.
%\filip{we have to add high-level guidance to the reader for this section. The reader has to know what is the relevance of each subsection. We could do this by pointing to the figure and explaining the coarse steps in a couple of sentences.}

\subsection{Task Definition}
\label{subsec:task1}
\textbf{Procedural text understanding} Given a paragraph $P = \{s_1, s_2, ... s_n\}$ consisting of n sentences, and a set of k entities $\{E_1, E_2, ... E_k\}$. The task is to predict precondition state $S_{it}^p$ and effect state, $S_{it}^e \in $\{\textit{non-existence}, \textit{unknown-location}, \textit{location}\} for every entity at every step,  where $i \in \{1,2,..k\}, t \in \{1,2,...n\}$. For \textit{location}, a span of text in $P$ needs be identified for the prediction. Here, the effect state at step t-1 is the same as precondition state at step t, i.e. $ S_{it-1}^e = S_{it}^p$, hence the $S_i$ can be viewed as a sequence of length n+1.\filip{this past sentence is hard to understand}
Additionally, the model needs to predict the action $A_{it} \in$ \{Create, Exist, Move, Destroy\} performed by the entity at every step. Here the action $A_{it}$ describes the entity state changes from precondition to effect, thus it can be inferred from the state sequence $S_i$. For example, if $S_{i1}^p =$ non-existence and $S_{i1}^e =$ location, then $A_{i1} =$ Create. Conversely, the state sequence can also be inferred from action sequence combined with the predicted locations, e.g. if $A_{i1} =$ Destroy then  $S_{i1}^p =$ location/unknown-location and $S_{i1}^e =$ non-existence. 
\filip{this subsection is fine, but maybe it can be improved by going from general info (there are entities, states and actions) to specific info (what are the states, how you transition, etc.)}

\textbf{Story Understanding}
Given two stories, $P_1$, $P_2 = \{s_1, s_2, ... s_n\}$ each consisting of n sentences, where only one of the sentences differ. The task is to identify which story is more plausible, and identify the conflicting pair of sentences ($s_{c1}$ and $s_{c2}$) in the implausible story. Additionally, the model needs to track the precondition $ S_{i}^e$ and effects $S_{i}^p$ of all entities at every step in each story, similar to \S\ref{subsec:task1}. In the task we consider, there are multiple dimensions of precondition and effect states, i.e. different attributes, all of which are defined in a discrete space. Also, the effect state at step t-1 no longer match precondition state at step t, hence $S_{it-1}^e \neq S_{it}^p$. 

\begin{figure*}
    \centering
    \includegraphics[scale=0.4]{Our_model.png}
    \caption{An illustration of our proposed model}
    \label{fig:model}
\end{figure*}

\subsection{Input Representation}
\label{subsec:input}
We propose to build a unique input representation for every entity at each step and provide it access to the entire context, as it would allow greater modeling flexibility and enable span extraction for location prediction. Given an entity, we create a pseudo question $Q$ ``where is \{entity\}'' , and concatenate it with the full paragraph $P$, resulting in $C$ = [CLS] $Q$ [SEP] $P$ [SEP]. We project $C$ it in the embedding space using an LM encoder's embedding layer, resulting in $C_{emb}$. We combine $C_{emb}$ with timestep embeddings to mark the current step of interest following \cite{rajaby-faghihi-kordjamshidi-2021-time}. Each input token is assigned a timestep id $T \in$\{0 = padding, 1 = past, 2 = current, 3 = future\} and the timestep sequence is projected through another embedding layer $Timestep \in \mathbb{R}^{4 \times d}$. The sum of $C_{emb}$ and $Timestep(T)$, denoted with $C_{emb}' \in \mathbb{R}^{m \times d}$, are then processed by the LM encoder, where $m$ is the number of tokens and $d$ is the hidden layer dimension of the LM encoder. Formally:

\begin{align}
    C_{emb} & = Embed(C) \\
    C_{emb}' & = C_{emb} + Timestep(T) \\
    C_{enc} & = LM Encoder(C_{emb}')
\end{align}
Note that we also build a input sequence for step 0 for every entity because we need to model the precondition state of step 1, i.e., the location span prediction. Thus the total number of input representation of an entity is n+1. \filip{ok, but shouldn't this also be mentioned in 2.1?}
\subsection{Location Prediction}
Given the encoded representation $C_{enc} \in \mathbb{R}^{m \times d}$ produced by the LM encoder, we extract the start and end indices of the location span. Formally, 
\begin{align}
    P_{Start} & = Softmax(W^T_s C_{enc})  \\
    P_{End} & = Softmax(W^T_e C_{enc}) 
\end{align}
where $W^T_s,W^T_e \in \mathbb{R}^{d}$. For unknown locations and non-existing states, we extract the [CLS] token as the span, analogous to how the unanswerable questions are handled in the literature \cite{rajpurkar-etal-2018-know}.

\subsection{In-batch CRF}
For entity state/action modeling, we propose to jointly predict the entity actions across all steps. We first group the encoded representation $C_{enc}^t$ of the same entity at different time steps $t$ in one batch chronically, yield $C_{enc}^N \in \mathbb{R}^{(n+1) \times m \times d}$. Then we extract the [CLS] token embedding to represent the entity state of every step $C_{enc}^{N'} \in \mathbb{R}^{(n+1) \times d}$. We concatenate the entity state representation of every two consecutive steps to represent the actions between these two-state pairs. The result $D_{enc}^{N} \in \mathbb{R}^{n \times 2d}$ is mapped to the emission probability $\phi \in \mathbb{R}^{n \times a}$, where a is the number of possible actions. Formally:
\begin{align}
    D_{enc}^t & = Concat(C_{enc}^{t'}, C_{enc}^{(t+1)'}) \\
    \phi & = W^T_a (tanh (W^T_d D_{enc}^{N}))
\end{align}
where  $W^T_d \in \mathbb{R}^{2d \times d}$, $W^T_a \in \mathbb{R}^{d \times a}$. The entity action sequence $A \in \mathbb{R}^{n}$ is modeled by a CRF layer, i.e.,
\begin{align}
    P(A|\phi, \psi) &  \propto \exp (\sum_{t=1}^{n} \phi_{t}(A_{t})+\psi(A_{t-1}, A_{t}))
\end{align}
where $\psi \in  \mathbb{R}^{a \times a}$ is the transition probability of the CRF layer. 

%P(\mathbf{y} \mid \mathbf{w}, e) \propto \exp \left(\sum_{i=0}^{T} \phi_{i}\left(y_{i}, \mathbf{w}, e\right)+\psi\left(y_{i-1}, y_{i}\right)\right)

\subsection{Prior Initialization}
\label{subsec:prior}
By default, the CRF transition probabilities are randomly initialized and updated during training, as done in previous works \cite{gupta-durrett-2019-tracking,zhang2021koala}. This indicates that the transition between any pair of actions is possible. However, certain transitions between entity actions are nonsensical, e.g., an entity cannot be destroyed if it has not been created and a destroyed cannot move. Given sufficient data, the model may be able to learn such knowledge eventually, however it is unlikely to have enough data for the tasks we are considering. Thus, we propose to directly impose these commonsense constraints on the model's transition probabilities, because these conditions are universally true and can be used to reduce the model's search space. Specifically, we set an entity action transition probability to 0 if it has not been seen in the training data, otherwise we estimate the initial probability of a transition based on its frequency in the training data:
\begin{align}
   \psi^{uv} & = log(\frac{Num(u, v)}{Num(u)})
\end{align}
Here, $\psi^{uv}$ is the transition probability from action $u$ to action $v$, $Num (u, v)$ is the count of transition from $u$ to $v$ in training data, $Num (u)$ is the count of $u$ in training data. % \filip{if this subsection is a novelty, we should emphasize that prior work does not do this. If it is not a novelty, we should point to prior work.}


\subsection{Training \& Inference}
\label{subsec:train}
We jointly optimize the location prediction loss and the entity action prediction loss during training:
\begin{align}
    \mathcal{L}_{loc} = - \frac{1}{n} \sum^{t=0}_n & (log(P_{Start}^{y_s^t}) + log(P_{End}^{y_e^t}))  \\
    \mathcal{L}_{action} & = -log(P(A|\phi, \psi)) \\
    \mathcal{L} = & \mathcal{L}_{loc} + \mathcal{L}_{action}
\end{align}
Here, $y_s^t$ and $y_e^t$ are ground-truth start and end indices at step t, respectively. During inference, we use Viterbi decoding to produce the most likely entity action sequence and use the span extractor to find the most likely location at every step. We then combine the action sequence and location predictions to deterministically infer all the precondition and effect states. 
%We do not need any post-processing heuristics to fix any nonsensical predictions, as done in previous works \cite{tang-etal-2020-understanding-procedural,rajaby-faghihi-kordjamshidi-2021-time, zhang2021koala}. Since our proposed prior initialization has zero-out impossible transition's probabilities, our model would not break any commonsense constraints.
%\textcolor{blue}{AO: Is removing impossible transitions equal to not breaking any commonsense constraint? I don't think you have explicitly stated what these constraints are. I'd imagine that, in the probability distribution of predicted actions sequences, some out of the less likely ones \textit{may} break \textit{some} commonsense constraints.}

\subsection{Data Augmentation}
The procedural text understanding task requires dense annotation of entity states at every step, making it challenging and expensive to collect large scale data. To remedy the data sparsity issue, we propose a data augmentation method that could effectively leverage the unannotated paragraphs to enhance model's performance. In particular, we first train a model on the gold training set and then apply it to label the unannotated paragraphs, resulting a set of noisy examples. We then mix these examples with gold training data to train a second model. 

\filip{It is a little hard to imagine how all the pieces tie in together - at the beginning of sec2 i suggested relying on the figure 2, but now i see also that the figure ideally needs to be updated to match the writing better.}

\filip{the local vs global split is not clear in this section. It is not clear how this justifies the contribution above.}

%\section{Procedure-Aware Story Understanding}

%We develop a story understanding method that integrates the procedural understanding model described in the previous section.

%\subsection{Task Definition}


\subsection{Model Adaptation}
\label{subsec:adapt}
We propose minimum modifications to our procedural text understanding model to apply it to the story understanding task. We first remove the span extraction layer and then on the input level, we no longer need step 0 input representation as location span prediction is not needed. Consequently, we directly use $C_{enc}^{N'} \in \mathbb{R}^{n \times d}$ instead of $D_{enc}^{N} \in \mathbb{R}^{n \times 2d}$ in the in-batch CRF, because the continuity of effects to preconditions between consecutive steps does not hold in this task. Given $B$ number of attributes for precondition and effect states, we propose to apply an in-batch CRF module for each attribute. Specifically, we apply equation 6 and 7 for every attribute and in total we have $2B$ such modules. 
For conflict sentences detection, we propose to concatenate every pair of sentence representations and pass through a linear layer to find the conflicting pair. For story classification, we take the mean of sentence representations for story representation, and pass through a linear layer for binary classification. Formally, \begin{align}
   C_{confl} & = vstack(Concat(C_{enc}^{t'}, C_{enc}^{j'})) \\
   P_{confl} & = Softmax(W^T_{confl} C_{confl}) \\
   C_{plau} & = Mean(C_{enc}^{N'}) \\
   P_{plau} & = Softmax(W^T_{plau} C_{plau}) 
\end{align}
where $C_{confl} \in \mathbb{R}^{\frac{n(n-1)}{2} \times d}$, $j \in \{{t+1},...n\}$, $W_{confl} \in \mathbb{R}^{d \times 1}$, $C_{plau} \in \mathbb{R}^{d \times 1}$, $W_{plau} \in \mathbb{R}^{d \times 2}$. Since each entity would produce prediction logits for conflict sentence pair and story plausibility, we take the average of all entities' logits as the final predictions. During training, we jointly optimize all three task objectives:
\begin{align}
    \mathcal{L}_{att} & = -log(P(S^{p}|\phi^{p}, \psi^{p}))-log(P(S^{e}|\phi^{e}, \psi^{e}))\\
   \mathcal{L} = & \mathcal{L}_{plau} + \mathcal{L}_{confl} + \frac{1}{B} \sum^{b=0}_B \mathcal{L}_{att}^b
\end{align}
